Randomized Block Coordinate Descent for Online and Stochastic Optimization

Two types of low cost-per-iteration gradient descent methods have been extensively studied in parallel. One is online or stochastic gradient descent (OGD/SGD), and the other is randomzied coordinate descent (RBCD). In this paper, we combine the two types of methods together and propose online randomized block coordinate descent (ORBCD). At each iteration, ORBCD only computes the partial gradient of one block coordinate of one mini-batch samples. ORBCD is well suited for the composite minimization problem where one function is the average of the losses of a large number of samples and the other is a simple regularizer defined on high dimensional variables. We show that the iteration complexity of ORBCD has the same order as OGD or SGD. For strongly convex functions, by reducing the variance of stochastic gradients, we show that ORBCD can converge at a geometric rate in expectation, matching the convergence rate of SGD with variance reduction and RBCD.

==> bcd.tex <==
% block coordinate descent 
In recent years, gradient descent and coordinate descent methods are the two most widely used algorithms in solving large scale machine learning problems due to their simplicity and scalability. They have been rigorously studied in both theory and applications~\cite{}. The randomized variants of two type algorithms, i.e., online/stochastic gradient descent and randomized coordinate descent methods, have particularly received lots of interests due to their low per-iteration cost. In particular, (block) coordinate descent methods have been studied under two types of rules. One is Guass-Seidel rule which updates coordinates in a cyclic order. The other is Jacobi rule which updates coordinates in parallel.  

In particular, the convergence of cyclic coordinate descent has been studied and linear convergence rate was established, but the iteration complexity of coordinate descent solving inexact minizmiation, like gradient descent, has been studied recently.  randomized coordinate gradient descent has been stuidied.  ~\cite{rita13:pbcd},~\cite{rita12:rbcd},~\cite{nesterov10:rbcd}.
Block coordinate descent methods have recently become very popular due to their low per-iteration cost and good scalability properties. While convergence results were established several decades ago, iteration complexity bounds were not studied until recently~\cite{tseng01:ds}.  
Randomized coordinate descent and block coordinate descent methods were proposed and analyzed in several settings, such as for smooth convex optimization problems~\cite{nesterov10:rbcd,rita12:rbcd}, $\ell_1$ regularized problems~\cite{shte09:sgd}.
block coordinate descent (BCD) methods have become very popular due to their low per-iteration complexity and scalability properties. While convergence results were established several decades ago, iteration complexity bounds were not studied until recently. 
randomized block coordinate descent~\cite{bkbg11:pbcd,rita13:pbcd,rita12:rbcd,nesterov10:rbcd}. ~\cite{luxiao13:rbcd}. 

==> theory.tex <==
The following lemma is a key building block of the proof of the convergence of OROLBCD in both online and stochastic setting.
\begin{lem}
Let $\x^t$ be the sequences generated by ORBCD. $j_t$ is sampled randomly and uniformly from $\{1,\cdots, J \}$. We have
\begin{align}\label{eq:orbcd_key_lem}
& \langle \nabla_{j_t} f_t(\x^t) + g'_{j_t}(\x_{j_t}^t), \x_{j_t}^{t} - \x_{j_t} \rangle   \leq \frac{\eta_t}{2} ( \| \x - \x^t \|_2^2 - \| \x - \x^{t+1} \|_2^2)  +  \frac{R^2}{2(\eta_t - L)}   + g(\x^t) - g(\x^{t+1})  ~.
\end{align}
where $L = \max_k L_k, R^2 = 2(R_f^2 + (J-1)R_g^2)$.
\end{lem}
\proof
The optimality condition is
\begin{align}
\langle \nabla_{j_t} f_t(\x^t) + \eta_t (\x_{j_t}^{t+1} - \x_{j_t}^t) + g'_{j_t}(\x_{j_t}^{t+1}),  \x_{j_t}^{t+1} - \x_{j_t} \rangle \leq 0~.
\end{align}
%Using the convexity of $g$, we have
%\begin{align}
%\langle \nabla_{j_t} f_t(\x^t) + \eta_t (\x_{j_t}^{t+1} - \x_{j_t}^t),  \x_{j_t}^{t+1} - \x_{j_t} \rangle + g_{j_t}(\x_{j_t}^{t+1}) - g_{j_t}(\x_{j_t}) \leq 0~.
%\end{align}
Rearranging the terms yields
\begin{align}
& \langle \nabla_{j_t} f_t(\x^t) + g'_{j_t}(\x_{j_t}^{t+1}) ,  \x_{j_t}^{t+1} - \x_{j_t} \rangle  \leq - \eta_t \langle  \x_{j_t}^{t+1} - \x_{j_t}^t ,  \x_{j_t}^{t+1} - \x_{j_t} \rangle \nonumber \\
& \leq \frac{\eta_t}{2} ( \| \x_{j_t} - \x_{j_t}^t \|_2^2 - \| \x_{j_t} - \x_{j_t}^{t+1} \|_2^2 - \| \x_{j_t}^{t+1} - \x_{j_t}^t \|_2^2 ) \nonumber \\
& = \frac{\eta_t}{2} ( \| \x - \x^t \|_2^2 - \| \x - \x^{t+1} \|_2^2 - \| \x_{j_t}^{t+1} - \x_{j_t}^t \|_2^2 )  ~,
\end{align}
where the last equality uses $\x^{t+1} = (\x_{j_t}^{t+1}, \x_{k\neq {j_t}}^t)$.
By the smoothness of $f_t$, we have
\begin{align}
f_t(\x^{t+1}) \leq f_t(\x^t) + \langle \nabla_j f_t(\x^t), \x_j^{t+1} - \x_j^t \rangle + \frac{L_j}{2} \| \x_j^{t+1} - \x_j^t \|_2^2~.
\end{align}
Since $\x^{t+1}  - \x^t = U_{j_t}(\x_{j_t}^{t+1} - \x_{j_t}^{t})$, the convexity of $g$ gives
\begin{align}
& g(\x^{t+1}) - g(\x^t) \leq \langle g'(\x^{t+1}), \x^{t+1} - \x^t \rangle \leq \langle g'_{j_t}(\x_{j_t}^{t+1}) + \sum_{\mathbb{I}_{j_t} \cap \mathbb{I}_k \neq \emptyset} g'_{k}(\x_{k}^{t+1}), \x_{j_t}^{t+1} - \x_{j_t}^t \rangle \nonumber \\
& \leq \langle g'_{j_t}(\x_{j_t}^{t+1}) , \x_{j_t}^{t+1} - \x_{j_t}^t \rangle + \frac{1}{2\alpha}\| \sum_{\mathbb{I}_{j_t} \cap \mathbb{I}_k \neq \emptyset} g'_{k}(\x_{k}^{t+1}) \|_2^2 + \frac{\alpha}{2} \| \x_{j_t}^{t+1} - \x_{j_t}^t \|_2^2 \nonumber \\
& \leq \langle g'_{j_t}(\x_{j_t}^{t+1}) , \x_{j_t}^{t+1} - \x_{j_t}^t \rangle + \frac{(J-1)R_g^2}{2\alpha} + \frac{\alpha}{2} \| \x_{j_t}^{t+1} - \x_{j_t}^t \|_2^2~.
\end{align}
\iffalse
\begin{align}
g(\x^{t+1}) - g(\x^t) \leq \langle g'_{j_t}(\x_{j_t}^{t+1}) , \x_{j_t}^{t+1} - \x_{j_t}^t \rangle~.
\end{align}
\begin{align}
\| \x_{k}^{t+1} - \x_{k}^t \|_2^2 = \| \x_{\mathbb{I}_{j_t} \cap \mathbb{I}_k \neq \emptyset}^{t+1} - \x_{\mathbb{I}_{j_t} \cap \mathbb{I}_k \neq \emptyset}^t \|_2^2 \leq \| \x_{j_t}^{t+1}  - \x_{j_t}^t \|_2^2~.
\end{align}
\begin{align}
\langle \sum_{\mathbb{I}_{j_t} \cap \mathbb{I}_k \neq \emptyset} g'_{k}(\x_{k}^{t+1}), \x_{k}^{t+1} - \x_{k}^t \rangle \leq \frac{(J-1)R_g^2}{2\alpha}  + \frac{\alpha}{2} \| \x_{j_t}^{t+1} - \x_{j_t}^t \|_2^2~.
\end{align}
\fi
Adding them together yields
\begin{align}
& f_t(\x^{t+1}) + g(\x^{t+1}) - [f_t(\x^t) + g(\x^t)] \nonumber \\
& \leq \langle \nabla_{j_t} f_t(\x^t), \x_{j_t}^{t+1} - \x_{j_t}^t \rangle + \frac{L_{j_t}}{2} \| \x_{j_t}^{t+1} - \x_{j_t}^t \|_2^2 + \langle g'_{j_t}(\x_{j_t}^{t+1}) , \x_{j_t}^{t+1} - \x_{j_t}^t \rangle + \frac{(J-1)R_g^2}{2\alpha} + \frac{\alpha}{2} \| \x_{j_t}^{t+1} - \x_{j_t}^t \|_2^2 \nonumber \\
& = \langle \nabla_{j_t} f_t(\x^t) + g'_{j_t}(\x_{j_t}^{t+1}), \x_{j_t}^{t+1} - \x_{j_t} \rangle +  \frac{L_{j_t}}{2} \| \x_{j_t}^{t+1} - \x_{j_t}^t \|_2^2  - \langle \nabla_{j_t} f_t(\x^t) + g'_{j_t}(\x_{j_t}^{t}), \x_{j_t}^{t} - \x_{j_t} \rangle \nonumber \\
& + \frac{(J-1)R_g^2}{2\alpha}  + \frac{\alpha}{2} \| \x_{j_t}^{t+1} - \x_{j_t}^t \|_2^2 \nonumber \\
& \leq \frac{\eta_t}{2} ( \| \x - \x^t \|_2^2 - \| \x - \x^{t+1} \|_2^2) +  \frac{L_{j_t} - \eta_t}{2} \| \x_{j_t}^{t+1} - \x_{j_t}^t \|_2^2 - \langle \nabla_{j_t} f_t(\x^t) + g'_{j_t}(\x_{j_t}^{t}), \x_{j_t}^{t} - \x_{j_t} \rangle \nonumber \\
& + \frac{(J-1)R_g^2}{2\alpha}  + \frac{\alpha}{2} \| \x_{j_t}^{t+1} - \x_{j_t}^t \|_2^2~.
\end{align}
Rearranging the terms yields
\begin{align}\label{eq:lem1}
& \langle \nabla_{j_t} f_t(\x^t) + g_{j_t}'(\x^t) , \x_{j_t}^{t} - \x_{j_t} \rangle  \leq \frac{\eta_t}{2} ( \| \x - \x^t \|_2^2 - \| \x - \x^{t+1} \|_2^2) +  \frac{L_{j_t} - \eta_t}{2} \| \x_{j_t}^{t+1} - \x_{j_t}^t \|_2^2  \nonumber \\
&+  f_t(\x^t)  + g(\x^t)-  [ f_t(\x^{t+1}) + g(\x^{t+1}) ] + \frac{(J-1)R_g^2}{2\alpha}  + \frac{\alpha}{2} \| \x_{j_t}^{t+1} - \x_{j_t}^t \|_2^2~.
\end{align}
The convexity of $f_t$ gives
\begin{align}
f_t(\x^t) -  f_t(\x^{t+1})  \leq \langle \nabla f_t(\x^t) , \x^t -  \x^{t+1} \rangle =  \langle \nabla_{j_t} f_t(\x^t) , \x_{j_t}^t -  \x_{j_t}^{t+1} \rangle \leq \frac{1}{2\alpha} \| \nabla_{j_t} f_t(\x^t) \|_2^2 + \frac{\alpha}{2} \| \x_{j_t}^t -  \x_{j_t}^{t+1} \|_2^2~.
\end{align}
where the equality uses $\x^{t+1} = (\x_{j_t}^{t+1}, \x_{k\neq {j_t}}^t)$. Plugging into~\myref{eq:lem1}, we have
\begin{align}
& \langle \nabla_{j_t} f_t(\x^t) + g'_{j_t}(\x_{j_t}^t), \x_{j_t}^{t} - \x_{j_t} \rangle   \nonumber \\
& \leq \frac{\eta_t}{2} ( \| \x - \x^t \|_2^2 - \| \x - \x^{t+1} \|_2^2) +  \frac{L_{j_t} - \eta_t}{2} \| \x_{j_t}^{t+1} - \x_{j_t}^t \|_2^2  +  \langle \nabla_{j_t} f_t(\x^t) , \x_{j_t}^t -  \x_{j_t}^{t+1} \rangle + g(\x^t) - g(\x^{t+1}) \nonumber \\
& + \frac{(J-1)R_g^2}{2\alpha}  + \frac{\alpha}{2} \| \x_{j_t}^{t+1} - \x_{j_t}^t \|_2^2 \nonumber \\
& \leq \frac{\eta_t}{2} ( \| \x - \x^t \|_2^2 - \| \x - \x^{t+1} \|_2^2) +  \frac{L_{j_t} - \eta_t}{2} \| \x_{j_t}^{t+1} - \x_{j_t}^t \|_2^2  + \alpha\| \x_{j_t}^t -  \x_{j_t}^{t+1} \|_2^2  \nonumber \\
& +  \frac{1}{2\alpha} \| \nabla_{j_t} f_t(\x^t) \|_2^2 + \frac{(J-1)R_g^2}{2\alpha}   + g(\x^t) - g(\x^{t+1})  ~.
\end{align}
Let $ L = \max_{k} L_k$. Setting $\alpha =\frac{ \eta_t - L}{2}$ where $\eta_t > L$ completes the proof.
\qed

This lemma is also a key building block in the proof of iteration complexity of GD, OGD/SGD and RBCD. In GD, by setting $\eta_t = L$, the iteration complexity of GD can be established. In RBCD, by simply setting $\eta_t = L_{j_t}$, the iteration complexity of RBCD can be established.

\subsection{Online Optimization}
Note $\x^t$ depends on the sequence of observed realization of the random variable 
$\xi_{t-1}^j = \{  j_1, \cdots, j_{t-1} \}$. 
The regret bound is defined as
\begin{align}
R(T) =  \sum_{t=1}^T\left \{ \mathbb{E}_{\xi_{t-1}^j}[ f_t(\x^t) + g(\x^t) ] - [f_t(\x) +g(\x)] \right \}~.
\end{align}
The following theorem establishes the regret bound of ORBCD.
\begin{thm}
Let $\eta_t = \sqrt{t} + L$ in the ORBCD.  $j_t$ is sampled randomly and uniformly from $\{1,\cdots, J \}$. The regret bound $R(T)$ of ORBCD is 
\begin{align}
R(T) \leq  J (  \frac{\sqrt{T} + L}{2}D^2 +  \sqrt{T} R^2 +   g(\x^1) - g(\x^*) )~.
\end{align}
\end{thm}
\proof
In~\myref{eq:orbcd_key_lem}, conditioned on $\x^t$, take expectation over $j_t$, we have
\begin{align}\label{eq:a}
\frac{1}{J}  \langle \nabla f_t(\x^t) + g'(\x^t), \x^{t} - \x \rangle  &\leq \frac{\eta_t}{2} ( \| \x - \x^t \|_2^2 - \mathbb{E}_{j_t}\| \x - \x^{t+1} \|_2^2)  +  \frac{R^2}{2(\eta_t - L)}  + g(\x^t) - \mathbb{E}_{j_t}g(\x^{t+1}) 
~.
\end{align}
Using the convexity, we have
\begin{align}
f_t(\x^t) + g(\x^t) - [f_t(\x) + g(\x)] \leq \langle \nabla f_t(\x^t) + g'(\x^t), \x^{t} - \x \rangle~.
\end{align}
Together with~\myref{eq:a}, we have
\begin{align}
f_t(\x^t) + g(\x^t) - [f_t(\x) + g(\x) ]   &\leq J \left \{ \frac{\eta_t}{2} ( \| \x - \x^t \|_2^2 - \mathbb{E}[\| \x - \x^{t+1} \|_2^2]) +  \frac{R^2}{2(\eta_t - L)} + g(\x^t) - \mathbb{E}g(\x^{t+1})  \right \}~.
\end{align}
Taking expectation over $\xi_{t-1}^j$ on both sides, we have
\begin{align}
\mathbb{E}_{\xi_{t-1}^j} \left [ f_t(\x^t) + g(\x^t) - [f_t(\x) + g(\x) ] \right ]   &\leq J \left \{ \frac{\eta_t}{2} ( \mathbb{E}_{\xi_{t-1}^j}\| \x - \x^t \|_2^2 - \mathbb{E}_{\xi_{t}}[\| \x - \x^{t+1} \|_2^2]) \right .\nonumber \\
& +  \left. \frac{R^2}{2(\eta_t - L)} + \mathbb{E}_{\xi_{t-1}^j} g(\x^t) - \mathbb{E}_{\xi_{t}}g(\x^{t+1})  \right \}~.
\end{align}
Summing over $t$ and setting $\eta_t = \sqrt{t} + L$, we obtain the regret bound
\begin{align}\label{eq:orbcd_rgt0}
& R(T) = \sum_{t=1}^T\left \{ \mathbb{E}_{\xi_{t-1}^j}  [ f_t(\x^t) + g(\x^t) ] - [f_t(\x) +g(\x)] \right \} \nonumber \\
&\leq J \left \{ - \frac{\eta_{T}}{2} \mathbb{E}\| \x - \x^{T+1} \|_2^2  + \sum_{t=1}^{T}(\eta_{t} - \eta_{t-1}) \mathbb{E}[\| \x - \x^{t} \|_2^2] +  \sum_{t=1}^{T}\frac{R^2}{2(\eta_t - L)}  + g(\x^1) - \mathbb{E}g(\x^{T+1}) \right \} \nonumber \\
& \leq J \left \{  \frac{\eta_T}{2} D^2  +  \sum_{t=1}^{T}\frac{R^2}{2(\eta_t - L)} +   g(\x^1) - g(\x^*) \right \}  \nonumber \\
& \leq J \left \{ \frac{\sqrt{T} + L}{2} D^2  +  \sum_{t=1}^{T}\frac{R^2}{2\sqrt{t} } + g(\x^1) - g(\x^*) \right \} \nonumber \\
& \leq  J (  \frac{\sqrt{T} + L}{2} D^2+  \sqrt{T} R^2 +   g(\x^1) - g(\x^*) )~,
\end{align}
which completes the proof.
\qed

If one of the functions is strongly convex, we have
\begin{align}\label{eq:stronggcov}
f_t(\x) + g(\x) \geq f_t(\x^t)  + g(\x^t) + \langle \nabla f_t(\x^t) + g'(\x^t), \x - \x^{t} \rangle +  \frac{\gamma}{2}  \| \x - \x^t \|_2^2~.
\end{align}
where $\gamma > 0$. ORBCD can still achieve a $\log(T)$ regret bound, which is established in the following theorem.
\begin{thm}\label{thm:orbcd_rgt_strong}
For strongly convex function, setting $\eta_t = \frac{\gamma t}{J} + L$ in the ORBCD. $j_t$ is sampled randomly and uniformly from $\{1,\cdots, J \}$. The regret bound $R(T)$ of ORBCD is 
\begin{align}
R(T) \leq   J^2R^2 \log(T) +   J(g(\x^1) - g(\x^*) ) ~.
\end{align}
\end{thm}
\proof
Using the strong convexity of $f_t + g$ in~\myref{eq:stronggcov}, we have
\begin{align}
f_t(\x^t) + g(\x^t) - [f_t(\x) + g(\x)] \leq \langle \nabla f_t(\x^t) + g'(\x^t), \x^{t} - \x \rangle - \frac{\gamma}{2} \| \x - \x^t \|_2^2~.
\end{align}
Together with~\myref{eq:a}, we have
\begin{align}
f_t(\x^t) + g(\x^t) - [f_t(\x) + g(\x) ]   &\leq \frac{J\eta_t - \gamma }{2} \| \x - \x^t \|_2^2 - \frac{J\eta_t}{2} \mathbb{E}[\| \x - \x^{t+1} \|_2^2]) \nonumber \\
& +  \frac{JR^2}{2(\eta_t - L)} + J [ g(\x^t) - \mathbb{E}g(\x^{t+1}) ] ~.
\end{align}
Taking expectation over $\xi_{t-1}^j$ on both sides, we have
\begin{align}
\mathbb{E}_{\xi_{t-1}^j} \left [ f_t(\x^t) + g(\x^t) - [f_t(\x) + g(\x) ] \right ]   &\leq \frac{J\eta_t - \gamma}{2} \mathbb{E}_{\xi_{t-1}^j}\| \x - \x^t \|_2^2 - \frac{J\eta_t}{2}\mathbb{E}_{\xi_{t}}[\| \x - \x^{t+1} \|_2^2]) \nonumber \\
& +   \frac{JR^2}{2(\eta_t - L)} + J [ \mathbb{E}_{\xi_{t-1}^j} g(\x^t) - \mathbb{E}_{\xi_{t}}g(\x^{t+1})  ]~.
\end{align}
Summing over $t$ and setting $\eta_t = \frac{\gamma t}{J} + L$,  we obtain the regret bound
\begin{align}
& R(T) = \sum_{t=1}^T\left \{ \mathbb{E}_{\xi_{t-1}^j}  [ f_t(\x^t) + g(\x^t) ] - [f_t(\x) +g(\x)] \right \} \nonumber \\
&\leq   - \frac{J\eta_{T}}{2} \mathbb{E}\| \x - \x^{T+1} \|_2^2  + \sum_{t=1}^{T}\frac{J\eta_{t} -\gamma - J\eta_{t-1}}{2}\mathbb{E}[\| \x - \x^{t} \|_2^2] +  \sum_{t=1}^{T}\frac{JR^2}{2(\eta_t - L)}  + J ( g(\x^1) - \mathbb{E}g(\x^{T+1}) ) \nonumber \\
& \leq \sum_{t=1}^{T}\frac{J^2R^2}{2\gamma t } +   J(g(\x^1) - g(\x^*) )  \nonumber \\
& \leq J^2R^2 \log(T) +   J(g(\x^1) - g(\x^*) )  ~,
\end{align}
which completes the proof.
\qed

In general, ORBCD can achieve the same order of regret bound as OGD and other first-order online optimization methods, although the constant could be $J$ times larger.

If setting $f_t = f$, OROLBCD turns to batch optimization or randomized overlapping block coordinate descent (ROLBCD). By dividing the regret bound by $T$ and denoting $\bar{\x}^T = \frac{1}{T}\sum_{t=1}^{T} \x^t$, we obtain the iteration complexity of ROLBCD, i.e.,
\begin{align}
\mathbb{E}_{\xi_{T-1}^j}[ f(\bar{\x}^T) + g(\bar{\x}^T) ] - [f(\x) +g(\x)] = \frac{R(T)}{T} ~.
\end{align}
The iteration complexity of ROLBCD is $O(\frac{1}{\sqrt{T}})$, which is worse than RBCD.
